Engineering Human Values in Software through Value Programming

Ignoring human values in software development may disadvantage users by breaching their values and introducing biases in software. This can be mitigated by informing developers about the value implications of their choices and taking initiatives to account for human values in software. To this end, we propose the notion of Value Programming with three principles: (P1) annotating source code and related artifacts with respect to values; (P2) inspecting source code to detect conditions that lead to biases and value breaches in software, i.e., (P3) making recommendations to mitigate biases and value breaches. To facilitate value programming, we propose a framework that allows for automated annotation of software code with respect to human values. The proposed framework lays a solid foundation for inspecting human values in code and making recommendations to overcome biases and value breaches in software.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile/.tex/.pdf}; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex $(notdir $<)
	cd $(dir $@) && pdflatex $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex $(notdir $<)
	cd $(dir $@) && xelatex $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*


==> limitations.tex <==
When Not To Use Annotations
Do not heavily use Annotation, since it will look dense and it can populate the code.
Do not try to change the behavior of Object using Annotation.
Code is the real PROGRAM and annotation is the META. So do not try to over generalize as it may complicate the code.
Do not use when dealing with database information.


==> motivation.tex <==
\section{Motivation}
\label{sec_motivation}
%
%As the bond between human and software grows stronger, considering human values in software systems design is becoming a priority for organizations, software users, and practitioners. But the available methods of engineering software are predominantly ignorant of such a need. 
%
%Traditional software engineering methods have mainly focused on timely delivery of functionality that adheres to acceptable levels of safety, privacy, and security. However, broader human values such as social justice and transparency remain under-represented in current software engineering methods. This can lead to breaching human values \cite{ferrario2016values} in software. Breaching values, however, may lead to dissatisfaction of the software users, lack of adoption, and devastating socio-economic repercussions such as loss of reputation and money. In the recent Volkswagen emissions fiasco, a deceptively designed software was installed to fool fuel emission tests. This was in clear contradiction to the company's corporate value of ``responsible thinking''. This decision led to the resignation of the Volkswagen CEO, a 30 percent drop in the company's stock price and a 25 percent drop in sales within a year \cite{kollewe_2016}. 
%
%Similarly, Galhotra et al.~\cite{Galhotra2017} cite other examples of `biased' software systems, which act in a way different to the values intended by their designers. For instance, Amazon's software for determining which US zip codes to give free same day shipping turned out to be biased against minority neighborhoods~\cite{gralla_2016}. Also, the risk-assessment systems of the US Justice Department have been proven to unfairly flag defendants of certain races as future criminals~\cite{angwin_larson_kirchner_mattu_2016}. Another example is the supply and demand software pricing systems that led to price gouging on airline tickets for those trying to evacuate from Hurricane Irma~\cite{sablich_2017} -- as the New York Times reported, ``There are no ethics valves built into the system that prevents an airline from overcharging during a hurricane.''
%
%There is a growing awareness of technology's impact on society; people are demanding that practitioners align technologies with human values. For example, Facebook's CEO was publicly scrutinized and questioned for allowing unauthorized use of users' personal data to influence the US elections \cite{smith_2018}. Similarly, Google has pledged its AI will no longer be used for weapons or surveillance that violates international norms or goes against human rights \cite{dave_2018}. These initiatives are welcome and are promising yet they are led by groups of AI researchers, not software engineering researchers or practitioners. It is time for a change in software engineering methods so that human values can be embedded in the software that society develops and uses. This paper thus presents a research roadmap for operationalizing human values in software -- that is, to integrate values into software in a verifiable way. %design and develop our capabilities to measure human values that exist in software. 
%
%%This paper, thus, aims to establish a research roadmap for overcoming these obstacles. The proposed roadmap focuses on (i) establishing practical definitions for human values, (ii) integrating values into software design, and (iii) measuring human values in software development life cycle. 
%
%
%
%%Some of these technology giants have recognized and begun to address these societal concerns. Companies like Microsoft, Amazon, Facebook, Apple, IBM, and DeepMind are partnering to study and define best practices for ensuring that the use of AI benefits society.

==> state.tex <==
\section{State of the Art}
\label{sec_related}

%\subsection{Human values in SE}
%\subsection{API-based analysis of security and privacy.}
%\subsection{API recommendation.}
%\subsection{Code smells and taint analysis.}

Human values are widely studies in social sciences~\cite{schwartz1992universals,schwartz1987toward,schwartz1994there,rokeach1973nature}. In this regard, Schwartz \cite{schwartz1992universals} introduced a universal model of human values based on studies across 68 societies (Table~\ref{schwartz1987toward}). 


The importance of considering human values in engineering software has been widely recognized~\cite{mougouei2018operationalizing}.  %Within and beyond software industry and research community, \textit{Value} is a multidimensional concept with overloaded words associated with it. In social sciences and physiology the plural term Values, also referred to as \textit{Human Values}, is widely adopted instead of \textit{value} to account for different types of human concerns and feelings \cite{schwartz1992universals,schwartz1987toward,schwartz1994there,rokeach1973nature}. In fact, in 1992, Schwartz introduced a substantial and universal model of human values \cite{schwartz1992universals} in which, 57 human values were categorized into 10 distinguishable types. 


 Nonetheless,  none of the existing works has addressed human values in software code. 

values have not yet successfully been translated into current software engineering practice.



%Contemporary attempts~\cite{koch2013approximate,harbers2015embedding,friedman2002value} to integrate human values in software have not lead to practical and verifiable solutions. Barn et al. \cite{barn2015role} highlighted this by stating: ``values have not yet successfully been translated into current software engineering practice.'' 
%
%We argue, in this paper, that the failure to integrate human values in software is mainly caused by (i) lack of practical definitions for human values in the field of software engineering, (ii) disregard of values in software design decisions, and (iii) lack of measurement of human values in software. 
%
%%---------------------------------------- Operationizable Model of Values ---------------------------------------------------------------------
%
%\textit{Lack of Practical Definitions for Values}. 
%The definitions of human values, e.g. fairness and social justice, vary depending on the context in which they apply \cite{kujala2008value}. For instance, consider \textit{security}: in a software engineering context, security mainly implies confidentiality, integrity, and availability in software while in a social-sciences context, security may manifest itself through concepts such as \textit{sense of belonging} and \textit{being healthy} (Figure~\ref{fig_values}). As such, a practical definition of a value should embody the meaning of that word in its corresponding socio-technical context \cite{friedman2013value}. To the best of our knowledge such definitions, for the majority of human values, do not exist in software engineering practice. %This is, clearly, a major obstacle in operationalizing human values in software. 
%
%%---------------------------------------- Values in Design Patterns ------------------------------------------------------------------------
%
%\textit{Overlooking Values in Design Decisions.} The majority of human values (Figure~\ref{fig_values}), except for the well-studied ones such as \textit{privacy}, have been overlooked when making decisions about designing software products. Having said that, we recognize the effort of individual software practitioners to account for human values. Such efforts, nevertheless, have not been formulated in a way they can be made available to other software practitioners, e.g. by integrating them into software design tools. An initiative \cite{friedman2013value} was undertaken by Friedman et al. to formulate theories for embedding values in information systems. The work, referred to as \textit{Value Sensitive Design} (VSD) \cite{friedman2013value}, emphasized adopting ``working'' definitions of human values and reconciling conflicting values, i.e. \textit{Value Tensions}. These are, however, missing from  existing software design methods. Furthermore, VSD has not been widely adopted by software practitioners. This might be due to the lack of sufficient traceability~\cite{aldewereld2015design}. 
%
%%These works further, ignore the value implications of commonly adopted software design practices, e.g. design patterns, which may therefore result in breaching (violating) human values in software. Several examples of such \textit{Value Breaches} have been described in the literature~\cite{Doty2013}. \hl{For example, using third-party passwords for a delegated authentication, instead of using protocols like \textit{open authentication} (OAuth) that enable delegated authorization, is a well-known example of a design practice that misaligns with privacy aspects of software and therefore can be identified as a privacy anti-pattern}~\cite{Doty2013}.
%
%%---------------------------------------- Measuring Values ---------------------------------------------------------------------
%
%\textit{Lack of Measurement of Human Values in Software.} Another important concern in operationalizing values in software is measuring and evaluating those values in software. This is essential to justify and evaluate decisions with respect to human values. A set of practical metrics, i.e. \textit{value metrics} are, therefore, required to measure the level of the presence or absence of human values at different stages of a software development life cycle. Without such metrics it would be hard, if possible at all, to trace the presence or absence of the values back to the design decisions. After years of research in software engineering, metrics have been developed for some of the human values, mainly the monetary values~\cite{biffl2006value} and the ones with clear ties to the well-explored quality aspects of software such as security and privacy~\cite{herrmann2007complete}. But software engineering, as a discipline, is still lacking metrics for the majority of the human values such as \textit{social and economic justice}, \textit{respect for tradition}, \textit{sense of belonging}, \textit{gender equality}, and so on. This might be due to the lack of sufficient attention paid to developing practical definitions for human values in software engineering practice.  
%
%
%
%
%
%\begin{figure*}[!htbp]
%	\centering
%	\centerline{\includegraphics[scale=0.802,angle=0]{figs/values}}
%	\captionsetup{margin=0.5cm}
%	\caption{Value Structure Across 68 Countries Based on Schwartz~\cite{schwartz2006valeurs,schwartz2004evaluating} (Adopted from \cite{ferrario2016values,holmes2011common}).}
%	\label{fig_values}
%\end{figure*}
%
%
%%Identification of Human Values for software systems is being studied for years, which result in different approaches, frameworks, methodologies and techniques. Most of them are coming form Requirement Engineering (RE) and Software Design. In RE, while some research works \cite{colomo2011using,koch2013approximate} contribute to this effort, Thew and Sutcliffe introduced a promising method \cite{thewvalue} that uses stakeholders' values, motivations and emotions with guidance for eliciting and analyzing soft-issues. Though the method identifies RE process management implications from values, it does not provide a proper guidance to covert identified human values to systems features \cite{harbers2015embedding}. Further, In software design, human values have extensively been studied and incorporated \cite{friedman1997human} through Human Computer Interaction (HCI) \cite{barn2015role,kujala2008value}. Value Sensitive Design (VSD) \cite{friedman2002value} a theoretically grounded approach to the design of technology that accounts for human values in a principled and comprehensive manner throughout the design process. 
%%
%%
%%by Friedman standouts among the rest of the HCI methods such as Participatory Design, Worth Centered Design and User-centered Design in terms of accounting and developing targeted methods for engaging \textit{human values} explicitly \cite{barn2015role, friedman2017survey,van2009value}. % Add main methodology for the VSD. A recent survey of VSD has discussed 14 invented methodologies which delivered VSD in addition to the general strategy of it \cite{friedman2017survey}. AOSE claim - no proper guidance to third step of the process 
%%However, translating identified human values into corresponding design features in the system is an underdeveloped activity in VSD \cite{harbers2015embedding,detweiler2011principles}. Therefore, in both promising works in RE and software Design, the observable problem is the inability to transform identified human values into implementable system features in a rational way. Thus, rather an informed guess, it requires a body of knowledge to address the logical sequence of such transformation that can answer \textit{what?},  \textit{how?} and \textit{why?} questions upon the software feature selections.  
%%Aldewereld and others have identified this problem and attempted solve it by introducing Value-Sensitive Software Development (VSSD) conceptual framework \cite{aldewereld2015design}. Admittedly, the work itself has emphasized the absence of procedures and guidelines to convert VSSD to a SE methodology in practice.  
%%
%%Over decades of research, some of the human values have overcome this problem by introducing proper metrics and matrices. Better examples would be the human values, with some monetary values \cite{biffl2006value} and the ones with clear ties to the well-explored quality aspects of software such as security and privacy\cite{galhotra2017fairness,herrmann2007complete}. But
%%the present software engineering, as a discipline, is severely lacking
%%metrics for the majority of human values such as social and
%%economic justice, respect for traditions, sense of belonging, gender
%%equality, and so on. In this regard, \cite{sutcliffe2014design} goes step further by identifying \textit{potential sources}, \textit{generic functional requirements} and \textit{architectural implications } for selected (commonly agreed in value theories) set of human values such as creativity, aesthetic, sociability, trust etc. For instance, \textit{extend able tools} were identified as a generic functional requirement for the value of \textit{creativity} while it generates an architectural implication as \textit{end-user development}. Further, \textit{Value Dams and Flows} method \cite{miller2007value} converts value concerns to functional requirements explicitly. For example, to secure the \textit{privacy} concerns of users, developers decided not to log \textit{who} searched the system while to secure the value of \textit{awareness} they logged the \textit{frequency} of item (code segment in this case) they searched. Unfortunately, these are either theoretical frameworks which in lack of empirical evidence to support with or emerged and validated through only a specific case study.
%%By introducing Values-First SE \cite{ferrario2016values}, Ferrario and others attempted to give more visibility to the interplay between SE choices and underlying human values. Barn and colleagues introduced  a framework \cite{barn2015role} to convert human values (again privacy and security) into SE practices. Admitting the lack of empirical evidence to support the framework, they recognized their research work as \textit{a call to
%%	arms and a vision for the SE community to recognize how systems impact on society at large}. In fact, they argued that \textit{values have not yet successfully been translated into current software engineering practice} though it appears in the design \cite{barn2015role}. 
%%
%%%It is evident through literature that, except for such scattered and isolated solutions, there is a huge research gap between human values and software implementation. A set of practical metrics, i.e. Value metrics are required not only for privacy or security but also for any human value in need. It allows to measure the presence or absence of human values in different stages of Software Development Life Cycle (SDLC) as
%%%well as the final product. Without such metrics, the presence or
%%%absence of human values in software neither can be verified nor
%%%can it be traced back to the design decisions and the efficiency of
%%%the techniques developed for engineering values in software, i.e.
%%%\textit{Valuefication Techniques}.
%%%% In addition, While VSD tends towards values with an ethical and social import, Ferrario et al. \textit{highlights the importance of a value mapping process that is independent from moral judgments} \cite{ferrario2016values,kujala2008value}. 
%%%% AOSE six principles - Make sure this aligns 
%%% \textbf{Representation}
%%%% Quality aspects - Non functional Requirements Vs. Values
%%%% Non functional requirements guidelines, standards, catalogue 
%%%% --- Find a suitable place to put this---
%%%%  Agile Developments and Value-based Software Engineering approaches address \textit{value(s)} as either pleasing customers or an economy/ROI related concern \cite{barn2015role,alahyari2017study}. Though both methodologies looks promising in integrating values, both are far removed from humane notion. Therefore we continued to search studies in SE that address human values explicitly. Surprisingly, there are only limited number of works which directly address human values through the software development methodology.
%%%%  ---------------
%%%
%%%In an effort to introduce more generic solutions in order to integrate human values into SE, design patterns step forward as a viable solution. In \cite{doty2013privacy} privacy design patterns were introduced as a remedy to lack of concrete guidance to implement \textit{Privacy-by-Design}. Similarly \cite{yoshioka2008survey} surveyed security design patterns. Works like these inflame the need of a generic model for design patterns for any human value(s) in need. In light of that, currently we are working on the \textit{concept of valufied design patterns} which is detailed in the next section of this paper. 
%%
%%
%%
%%%---------------------------------------------------------------------------------------------------------------------------------------------------
%%
%%
%%%Lack of an operationalizable representation of values that links them to their real-world manifestations in  software context seems to a major challenge here. 
%%
%%
%% 
%%%---------------------------------------------------------------------------------------------------------------------------------------------------
%%% Traceability of human values in software is another vacuum we identified which barely addressed by the SE as a discipline except for the well known privacy and security \cite{anthonysamy2012method}.  


